Area-preserving parameterizations for spherical ellipses

We present new methods for uniformly sampling the solid angle subtended by a disk. To achieve this, we devise two novel area-preserving mappings from the unit square $[0,1]^2$ to a spherical ellipse (i.e. the projection of the disk onto the unit sphere). These mappings allow for low-variance stratified sampling of direct illumination from disk-shaped light sources. We discuss how to efficiently incorporate our methods into a production renderer and demonstrate the quality of our maps, showing significantly lower variance than previous work.

==> src40_symboltable.tex <==
\begin{table}
	\centering
	\caption{\new{Notation used in this paper.}}
	\new{\begin{tabular}{ ll }
		\toprule
		\textbf{Symbol} & \textbf{Description} \\
		\midrule
		$\minorArc$, $\mayorArc$ & Major and minor semi-arcs of the spherical ellipse \\
		$\aplanar$, $\bplanar$ & Major and minor semi-axes of the spherical ellipse \\
		$\atang$, $\btang$ & Major and minor semi-axes of the tangent ellipse \\
		$\lightSolidAngle$ & Solid angle of the disk \\
		$\PartialSA(\gamma)$ & Partial solid angle of the spherical ellipse \\
		$\PartialHalfSA(\gamma)$ & Partial upper half solid angle of the spherical ellipse \\
		$\solidAngleRadial(\phi)$ & Partial solid angle of a spherical ellipse quadrant \\
		\toprule
	\end{tabular}}
	\iliyan{Let's remove this table, it's not really useful.}
\end{table}
\endinput

